Higher dimensional Reidemeister torsion invariants for cusped hyperbolic 3-manifolds

For an oriented finite volume hyperbolic 3-manifold M with a fixed spin structure \eta, we consider a sequence of invariants {\tau_n(M; \eta)}. Roughly speaking, {\tau_n(M; \eta)} is the Reidemeister torsion of M with respect to the representation given by the composition of the lift of the holonomy representation defined by \eta, and the n-dimensional, irreducible, complex representation of SL(2,C). In the present work, we focus on two aspects of this invariant: its asymptotic behavior and its relationship with the complex-length spectrum of the manifold. Concerning the former, we prove that for suitable spin structures, log(\tau_n(M; \eta)) grows as -n^2 Vol(M)/4\pi, extending thus the result obtained by W. Mueller for the compact case. Concerning the latter, we prove that the sequence {\tau_n(M; \eta)} determines the complex-length spectrum of the manifold up to complex conjugation.

==> spin.tex <==
\subsection{Lifts of the holonomy representation}
\label{subsection:lifts}

Let $M$ be a connected oriented hyperbolic $3$-manifold which is not necessarily complete.
The aim of this subsection is to review the relation between spin structures on $M$
and lifts of its holonomy representation to $\sln(2,\cmplx)$.
We will use the following definition of a spin structure, see \cite{Kirby}. 
The $\son(3)$-principal bundle of orthonormal positively oriented frames of $M$ is denoted by $P_{\son(3)} M$.

\begin{definition}
	A spin structure on $M$ is a (double) cover of $P_{\son(3)} M$ by a $\spin(3)$-principal bundle over $M$. 
\end{definition}

The above definition is equivalent to say that a spin structure on $M$ 
is a double cover of $P_{\son(3)} M$ such that the preimage of any fiber of $P_{\son(3)} M$ is connected.
It can be checked then that there is a natural identification between the set of spin structures on $M$ and the set
\[
\left \{ \alpha \in \cohom^1(P_{\son(3)} M; \modtwo) \mid i^*(\alpha) = 1 \in \cohom^1(\son(3); \modtwo) \right \}.
\]

On the other hand, the hyperbolic structure of $M$ defines a canonical flat $\Isom^+ \hyp^3$-principal bundle over $M$,
see \cite{Thurston3d}.
Let us recall how it is defined. Let $\hyp^3$ be hyperbolic space of dimension $3$ with a fixed orientation.
Consider an $(\Isom^+ \hyp^3, \hyp^3)$-atlas on $M$ defining the hyperbolic structure.
Thus we have local charts $\phi_i \colon U_i \to \hyp^3$ covering $M$
such that the changes of coordinates are restrictions of orientation preserving isometries of $\hyp^3$. 
We can assume that the local charts preserve the fixed orientations on both $M$ and $\hyp^3$.
Let $\psi_{ij}$ be the change of coordinates from 
$(\phi_j, U_j)$ to $(\phi_i, U_i)$, that is,
\[
\psi_{ij}\colon U_i\cap U_j \to \Isom^+ \hyp^3, \quad \psi_{ij} \circ \phi_j = \phi_i.
\]
The analyticity of the elements of $\Isom^+ \hyp^3$ implies that $\psi_{ij}$ is a locally constant map. 
Since these maps also satisfy the cocycle condition  
$\psi_{ij} \circ \psi_{jk} = \psi_{ik}$,
they define a flat $\Isom^+ \hyp^3$-principal bundle over $M$, 
\[ 
\Isom^+ \hyp^3 \to P_{\Isom^+ \hyp^3} M \overset{\pi}{\to} M.
\]
Let us fix a base point $p\in M$. Given $u\in P_{\Isom^+ \hyp^3} M$ with $\pi(u) = p$, 
it makes sense to consider the holonomy representation of this principal bundle,
\[
\Hol_u \colon \pi_1(M, p) \to \Isom^+ \hyp^3.
\]
Recall that, by definition, if $\sigma \colon [0,1] \to M$ is a loop based at $p$, 
$\Hol_u(\sigma)$ is the unique element of $\Isom^+ \hyp^3$ such that 
\[
\tilde{\sigma}(1) \cdot \Hol_u(\sigma) = \tilde{\sigma}(0),
\]
where $\tilde{\sigma}(t)$ is the horizontal lift of $\sigma(t)$ starting at $u$.
It can be checked that this holonomy is, up to a conjugation, the same as the one given in terms of the developing map.
In other words, for some suitable initial choices, we have $\Hol_u = \Hol_M$.

\begin{proposition} \label{prop: liftssl2}
	There is a canonical one-to-one correspondence between the following sets:
	\begin{enumerate}
		\item The set of covers of $P_{\psl(2,\cmplx)} M$ by $\sln(2,\cmplx)$-principal bundles over $M$. 
		\item The set of lifts of $\Hol_M$ to $\sln(2,\cmplx)$.
	\end{enumerate}
\end{proposition}
\begin{proof}
	Let us assume that we have chosen base points $p\in M$,
	$u\in P_{\psl(2,\cmplx)} M$ with $\pi(u) = p$, such that $\Hol_u = \Hol_M$.
	Let $P_{\sln(2,\cmplx)} M$ be an $\sln(2,\cmplx)$-principal bundle over $M$ covering 
	$P_{\psl(2,\cmplx)} M$. Take one of the two points 
	$\tilde{u} \in P_{\sln(2,\cmplx)}M$ that projects to $u$, and consider 
	the corresponding holonomy representation $\Hol_{\tilde{u}}$. 
	It is clear that $\Hol_{\tilde{u}}$ is a lift of $\Hol_u$; 
	moreover, it is independent of the choice of the base point $\tilde{u}$, 
	since the other choice is obtained by conjugating it by $-\operatorname{Id} \in \sln(2, \cmplx)$.
	This gives a well defined correspondence between 
	the set of covers of $P_{\psl(2,\cmplx)} M$ by $\sln(2,\cmplx)$-principal bundles over $M$
	and the set of lifts of $\Hol_M$ to $\sln(2,\cmplx)$.
	Since we can recover the flat bundle from its holonomy representation, this correspondence is one-to-one. 
\end{proof}

Next, we want to embed the frame bundle $P_{\son(3)} M$ into $P_{\psl(2,\cmplx)} M$.
To that end, identify $\psl(2,\cmplx)$ with $P_{\son(3)} \hyp^3$
by fixing a positively oriented frame $R_O \in P_{\son(3)} \hyp^3$.
Notice that it gives a concrete embedding of $\son(3)$ into $\psl(2,\cmplx)$.
Now let $u \in P_{\psl(2,\cmplx)} M$ and $p = \pi(u)$. 
Take a local chart $(\phi_j, U_j)$ of the hyperbolic structure with $p \in U_j$.
This gives a local trivialization $U_j \times G$ of $P_{\psl(2,\cmplx)} M$. 
Respect to this trivialization, the point $u$ is written as a pair $(p, g)\in U_j \times \psl(2,\cmplx)$. 
We will say that $u$ \emph{is based at} $p \in M$ , if $g \in \psl(2,\cmplx) \cong P_{\son(3)} \hyp^3$ 
is a frame based at $\phi_j(p)$. It can be checked that this definition does not 
depend on the choice of the local chart $(\phi_j, U_j)$. 
The following set is canonically identified with the bundle of positively oriented frames in $M$,
\[
\left \{ u \in P_{\Isom^+ \hyp^3} M \mid u \text{ is a frame based at } \pi(u)  \right \} \cong P_{\son(3)} M.
\]
This gives a concrete embedding $P_{\son(3)} M \hookrightarrow P_{\psl(2,\cmplx)} M $
(in other words, we have obtained an explicit reduction of the structural group respect to the fixed embedding $\son(3)\subset \psl(2,\cmplx)$).
Although the embedding just defined depends on the choices done, it must be pointed out that its homotopy class does not.

\begin{comment}
	A deformation retract is easily constructed as follows. 
	Let $u \in P_{\Isom^+ \hyp^3} M $, and write 
	it as $(p, g)$ using a trivialization relative to a local chart $(\phi, U)$. 
	Interpret $g$ as a frame on $\hyp^3$ based at a point 
	$q\in\hyp^3$, and let $\gamma\colon [0,1]\to \hyp^3$ the unique geodesic 
	such that $\gamma(0) = q$ and $\gamma(1) = \phi(p)$. 
	The parallel transport of $g$ along $\gamma$ yields a frame based at $p$. 
	This construction gives a well defined deformation retract
	$r_t \colon P_{\Isom^+ \hyp^3} M \to P_{\son(3)} M$.
\end{comment}

\begin{proposition}
	\label{prop:spin_lifts}
	There is a canonical one-to-one correspondence between the following sets:
	\begin{enumerate}
		\item The set of covers of $P_{\psl(2,\cmplx)} M$ by $\sln(2,\cmplx)$-principal bundles over $M$. 
		\item The set of spin structures on $M$.
	\end{enumerate}
\end{proposition}
\begin{proof}
	As we have observed, the set of spin structures on $M$ is canonically identified with 
	\[
	\left \{ \alpha \in \cohom^1(P_{\son(3)} M; \modtwo) \mid i^*(\alpha) = 1 \in \cohom^1(\son(n); \modtwo) \right \}.
	\]
	The same argument shows that the set of covers of $P_{\psl(2,\cmplx)} M$ by $\sln(2,\cmplx)$-principal bundles over $M$
	is identified with 
	\[
	\left \{ \alpha \in \cohom^1( P_{\psl(2,\cmplx)} M; \modtwo) \mid i^*(\alpha) = 1 \in \cohom^1(\sln(2,\cmplx); \modtwo) \right \}.
	\]
	The result then follows from the fact that the map $P_{\son(3)} M \hookrightarrow P_{\Isom^+ \hyp^3} M$ defined above,
	whose homotopy class is canonical, is a homotopy equivalence as $\son(3) \simeq \psl(2, \cmplx)$.
\end{proof}

\begin{corollary}
	The holonomy representation of a hyperbolic $3$-manifold 
	can be lifted to $\sln(2,\cmplx)$.
	The number of such lifts is $|\cohom^1(M;\modtwo)|$. 
\end{corollary}
\begin{proof}
	An oriented $3$-manifold admits $|\cohom^1(M;\modtwo)|$ 
	different spin structures.
\end{proof}

Next we want to prove the existence of acyclic spin structures on
an oriented complete hyperbolic $3$-manifold $M$ of finite volume.
Recall that a spin structure $\eta$ is acyclic if and only if $\cohom^0(T_i; \Hol_{(M,\eta)})$ is trivial 
for each connected component $T_i$ of the boundary.
Let us fix $T_i$, and denote it as $T^2$.
We can assume that $T^2$ is a horospheric cross-section, and that 
\[
\Hol_M (\pi_1 T^2) = \left \langle
	\left[ \begin{pmatrix}  
		1 & 1 \\ 
		0 & 1
	\end{pmatrix} \right], 
	\left[ \begin{pmatrix}  
		1 & \tau \\ 
		0 & 1
	\end{pmatrix} \right]
	\right \rangle < \psl(2, \cmplx), \quad \text{ with } \Im \tau > 0.
\]
Let $P_{\son(3)} T^2 \subset P_{\psl(2,\cmplx)} T^2$ be the restriction of 
$P_{\son(3)} M \subset P_{\psl(2,\cmplx)} M$ to $T^2$, and let $\Hol_{T^2}$ be the restriction of 
$\Hol_M$ to $\pi_1 T^2$.

Using the Euclidean structure of $T^2$ and the outward normal vector of $T^2$
we can construct a section $s$ of the bundle $P_{\son(3)} T^2$ that is canonical 
up to conjugation.
Indeed, fix $p \in T^2$ and define $s(p) \in P_{\son(3)} T^2$ 
as any frame based at $p$ whose third component is equal to the outward normal vector at $p$;
for $q \in T^2$, define $s(q)$ as the parallel transport (respect to the euclidean structure) of $s(p)$ along a curve joining $p$ and $q$ on $T^2$.
This yields a well defined section which is canonical up to homotopy.
Thus we have a canonical trivialization $P_{\son(3)} T^2 = T^2 \times \son(3)$,
and hence a distinguished spin structure $T^2 \times \spin(3)$.
All the others spin structures arise as quotients of the form
\[
\eta_{\alpha} = \left(\widetilde{T^2}\times \spin(3) \right) / \pi_1 T^2, 
\]
where $\alpha \in \cohom^1(T^2; \modtwo) = \operatorname{Hom}(\pi_1 T^2; \{ \pm 1\})$,
and $\sigma \in \pi_1 T^2$ acts on $\spin(3)$ by multiplication by $\alpha(\sigma) \operatorname{Id}$.
Therefore, spin structures of $P_{\son(3)} T^2$ are in canonical one-to-one correspondence with 
$\cohom^1(T^2;\modtwo)$.

Therefore, given $\alpha \in \cohom^1(T^2; \modtwo)$ we have also 
a cover of $P_{\psl(2,\cmplx)} T^2$ by an $\sln(2,\cmplx)$-principal bundle.
The above discussion shows that this is given by 
\[
\left(\widetilde{T^2}\times \sln(2, \cmplx) \right) / \pi_1 T^2,
\]
where $\sigma \in \pi_1 T^2$ acts on $\sln(2, \cmplx)$ by multiplication by $\alpha(\sigma) \operatorname{Id}$.
Taking this into account, the following result is easily proved.

\begin{lemma}
	Let $\alpha \in \cohom^1(T^2; \modtwo) = \operatorname{Hom}(\pi_1 T^2; \{ \pm 1\})$, $\eta_\alpha$ the associated spin structure on $T^2$,
	and $\Hol_{(T^2,\eta_\alpha)}$ the corresponding lift of the holonomy representation.
	Then we have
	\[
	\alpha(\sigma) = \operatorname{sgn} \tr \Hol_{(T^2,\eta_\alpha)}(\sigma), \quad\text{for all } \sigma \in \pi_1 T^2.
	\]
\end{lemma}
Now we can prove the existence of spin acyclic structures.
\begin{proposition} \label{prop:existenceacyclicspin}
	Let $M$ be an oriented complete hyperbolic $3$-manifold of finite volume.
	For each connected boundary component $T_i$ take a closed simple curve $\gamma_i$.
	Then there exists a spin structure $\eta$ on $M$ such that  
	\[
	\tr{\Hol_{(M, \eta)}} ( [\gamma_i]) = -2, 
	\]
	where $[\gamma_i]$ is the conjugacy class of $\pi_1 (M, p)$ defined by $\gamma_i$.
\end{proposition}
\begin{proof}
	Let $N$ be the manifold obtained by performing a Dehn filling along each 
	of the curves $\{\gamma_i\}$. Fix a spin structure $\eta$ on $N$.
	We claim that the restriction of $\eta$ to $M$ gives the required spin structure.

	Assume that $\gamma$ is one of the curves $\gamma_i$, and that it is contained in a horospheric cross-section $T^2$.
	For the sake of concreteness, assume also that $\gamma$ is a closed geodesic respect to the euclidean structure of $T^2$. 
	Let $P_{\spin(3)} T^2 \to P_{\son(3)} T^2$ the corresponding $\spin(3)$-bundle over $T^2$ defined by $\eta$.
	Consider the canonical section $s\colon T^2 \to P_{\son(3)} T^2$ constructed above using as starting frame one whose
	first vector is tangent to $\gamma$. Notice that the closed curve $s \circ \gamma$ can be lifted to $P_{\spin(3)} T^2$
	if and only if $\alpha(\gamma) = 1$. On the other hand, if $s \circ \gamma$ could be lifted to $P_{\spin(3)} T^2$,
	then such lift could be extended to added disk that bounds $\gamma$ 
	(as there is no obstruction in doing it, $\pi_1 \spin(3) = \{1\}$), and hence
	$s \circ \gamma$ could be extended to that disk, what is not possible by construction.
	Thus $\alpha(\gamma) = -1$, and the preceding lemma implies the result.
\end{proof}

As a corollary of the proof of the above proposition, we obtain the following result.
\begin{corollary} \label{coro:spinextension}
	Let $\eta$ be a spin structure on $M$. Let $\gamma \subset \partial M$ 
	be a simple closed curve non-homotopically trivial in $\partial M$,
	and $M_\gamma$ be the manifold obtained by performing a Dehn filling along $\gamma$.
	Then $\eta$ extends to a spin structure on $M_\gamma$ if and only if 
	$\Hol_{(M,\eta)} (\gamma)$ has trace $-2$.
\end{corollary}
The following corollary of Proposition \ref{prop:existenceacyclicspin} gives a sufficient condition that guarantees
the acyclicity of all spin structures.
\begin{corollary}
	Assume that for each connected boundary component $T_i$ of $M$, 
	the map $\cohom_1 (T_i; \modtwo) \to \cohom_1(M; \modtwo)$ induced by the inclusion has non-trivial kernel.
	Then all spin structures on $M$ are acyclic. 
	In particular, if $M$ has one cusp, all spin structures are acyclic.
\end{corollary}
\begin{proof}
	If the hypothesis holds, then for each $T_i$ there exists a closed simple curve $\gamma_i \in T_i$
	that is zero in $\cohom_1(M; \modtwo)$. Take a spin structure on $M$ such that
	$\tr{\Hol_{(M, \eta)}} ( [\gamma_i]) = -2$, for all $\gamma_i$. Now let $\eta'$ be another spin structure on $M$, 
	and $\alpha \in \cohom^1(M; \modtwo)$ the cohomology class relating $\eta$ and $\eta'$. Then, using multiplicative notation, we have
	\[
	\Hol_{(M, \eta')} ( \gamma_i) = \alpha(\gamma_i) \Hol_{(M, \eta)} ( \gamma_i). 
	\]
	Since $\alpha(\gamma_i) = 1$, $\Hol_{(M, \eta')} ( \gamma_i)$ has trace $-2$, as we wanted to prove.
	The rest of the result follows from the fact that in any compact $3$-manifold $M$ 
	the map $\cohom_1(\partial M; \modtwo) \to \cohom_1( M; \modtwo)$ induced by the inclusion has a
	non-trivial kernel.
\end{proof}

